Meta-Learning for Fast Cross-Lingual Adaptation in Dependency Parsing

Meta-learning, or learning to learn, is a technique that can help to overcome resource scarcity in cross-lingual NLP problems, by enabling fast adaptation to new tasks. We apply model-agnostic meta-learning (MAML) to the task of cross-lingual dependency parsing. We train our model on a diverse set of languages to learn a parameter initialization that can adapt quickly to new languages. We find that meta-learning with pre-training can significantly improve upon the performance of language transfer and standard supervised learning baselines for a variety of unseen, typologically diverse, and low-resource languages, in a few-shot learning setup.

==> content/tables/full_s20.tex <==
\begin{tabular}{l|cccccccc}\toprule
%& & & \multicolumn{3}{c|}{$|S|=20$} & \multicolumn{3}{c|}{$|S|=40$} & \multicolumn{3}{c}{$|S|=80$} \\
\textbf{Language} & \textbf{\textsc{en}} & \textbf{\textsc{hin}} & \textbf{\textsc{ne} (EN)} & \textbf{\textsc{ne} (HIN)} & \textbf{\textsc{maml}} & \textbf{\textsc{maml} (HIN)} & \textbf{\MAMLPrime}
\\ \midrule
\multicolumn{3}{l}{\textit{Low-Resource Languages}} & \multicolumn{5}{l}{} \\
Armenian  &   {49.80}{\scriptsize $\pm$0.005} & {48.41}{\scriptsize $\pm$0.002} & {63.34}{\scriptsize $\pm$0.002} & {63.30}{\scriptsize $\pm$0.005} & \bf {63.84}{\scriptsize $\pm$0.002} & {63.76}{\scriptsize $\pm$0.003} & {59.70}{\scriptsize $\pm$0.004} & \\
Breton  &   {60.34}{\scriptsize $\pm$0.003} & {34.06}{\scriptsize $\pm$0.005} & {61.44}{\scriptsize $\pm$0.005} & {62.09}{\scriptsize $\pm$0.004} & \bf {64.18}{\scriptsize $\pm$0.003} & {61.56}{\scriptsize $\pm$0.002} & {59.33}{\scriptsize $\pm$0.005} & \\
Buryat  &   {23.66}{\scriptsize $\pm$0.002} & {24.24}{\scriptsize $\pm$0.002} & {25.56}{\scriptsize $\pm$0.003} & {25.05}{\scriptsize $\pm$0.003} & {25.77}{\scriptsize $\pm$0.002} & \bf {26.27}{\scriptsize $\pm$0.002} & {26.02}{\scriptsize $\pm$0.004} & \\
Faroese  &   {68.50}{\scriptsize $\pm$0.004} & {50.72}{\scriptsize $\pm$0.004} & {67.83}{\scriptsize $\pm$0.006} & {65.31}{\scriptsize $\pm$0.006} & \bf {68.95}{\scriptsize $\pm$0.003} & {66.82}{\scriptsize $\pm$0.002} & {65.30}{\scriptsize $\pm$0.005} & \\
Kazakh  &   {47.25}{\scriptsize $\pm$0.004} & {49.80}{\scriptsize $\pm$0.002} & {55.02}{\scriptsize $\pm$0.002} & {53.77}{\scriptsize $\pm$0.003} & \bf {55.07}{\scriptsize $\pm$0.002} & {54.23}{\scriptsize $\pm$0.003} & {53.92}{\scriptsize $\pm$0.005} & \\
U.Sorbian  &   {49.29}{\scriptsize $\pm$0.004} & {36.22}{\scriptsize $\pm$0.003} & {54.47}{\scriptsize $\pm$0.003} & {53.36}{\scriptsize $\pm$0.003} & \bf {56.40}{\scriptsize $\pm$0.004} & {54.97}{\scriptsize $\pm$0.005} & {51.67}{\scriptsize $\pm$0.004} & \\
\midrule
\multicolumn{3}{l}{\textit{Unseen High-Resource Languages }} & \multicolumn{5}{l}{} \\
Finnish  &   {56.61}{\scriptsize $\pm$0.002} & {50.49}{\scriptsize $\pm$0.003} & \bf {64.94}{\scriptsize $\pm$0.003} & {64.05}{\scriptsize $\pm$0.004} & {64.89}{\scriptsize $\pm$0.003} & {64.64}{\scriptsize $\pm$0.002} & {61.97}{\scriptsize $\pm$0.005} & \\
French  &   {65.21}{\scriptsize $\pm$0.001} & {31.16}{\scriptsize $\pm$0.003} & {66.55}{\scriptsize $\pm$0.001} & {64.44}{\scriptsize $\pm$0.002} & \bf {66.85}{\scriptsize $\pm$0.001} & {65.73}{\scriptsize $\pm$0.001} & {63.42}{\scriptsize $\pm$0.003} & \\
German  &   {72.47}{\scriptsize $\pm$0.001} & {44.83}{\scriptsize $\pm$0.004} & {76.15}{\scriptsize $\pm$0.002} & {74.40}{\scriptsize $\pm$0.002} & \bf {76.41}{\scriptsize $\pm$0.002} & {75.15}{\scriptsize $\pm$0.001} & {74.38}{\scriptsize $\pm$0.003} & \\
Hungarian  &   {56.50}{\scriptsize $\pm$0.003} & {46.72}{\scriptsize $\pm$0.004} & \bf {62.93}{\scriptsize $\pm$0.003} & {60.98}{\scriptsize $\pm$0.002} & {62.71}{\scriptsize $\pm$0.003} & {62.51}{\scriptsize $\pm$0.004} & {58.47}{\scriptsize $\pm$0.002} & \\
Japanese  &   {18.87}{\scriptsize $\pm$0.002} & {40.25}{\scriptsize $\pm$0.005} & {36.49}{\scriptsize $\pm$0.008} & {39.97}{\scriptsize $\pm$0.003} & {39.06}{\scriptsize $\pm$0.003} & \bf {41.96}{\scriptsize $\pm$0.005} & {39.72}{\scriptsize $\pm$0.007} & \\
Persian  &   {43.43}{\scriptsize $\pm$0.005} & {28.60}{\scriptsize $\pm$0.004} & {52.55}{\scriptsize $\pm$0.006} & \bf {53.73}{\scriptsize $\pm$0.004} & {52.81}{\scriptsize $\pm$0.005} & {53.63}{\scriptsize $\pm$0.003} & {50.31}{\scriptsize $\pm$0.004} & \\
Swedish  &   {80.26}{\scriptsize $\pm$0.001} & {46.96}{\scriptsize $\pm$0.004} & {80.73}{\scriptsize $\pm$0.001} & {79.24}{\scriptsize $\pm$0.002} & \bf {81.36}{\scriptsize $\pm$0.001} & {79.89}{\scriptsize $\pm$0.001} & {77.57}{\scriptsize $\pm$0.002} & \\
Tamil  &   {31.58}{\scriptsize $\pm$0.005} & {46.51}{\scriptsize $\pm$0.003} & {41.12}{\scriptsize $\pm$0.009} & {39.44}{\scriptsize $\pm$0.006} & {44.34}{\scriptsize $\pm$0.005} & {39.57}{\scriptsize $\pm$0.008} & \bf {46.55}{\scriptsize $\pm$0.001} & \\
Urdu  &   {25.71}{\scriptsize $\pm$0.004} & \bf {67.72}{\scriptsize $\pm$0.001} & {57.25}{\scriptsize $\pm$0.004} & {50.64}{\scriptsize $\pm$0.004} & {55.16}{\scriptsize $\pm$0.004} & {49.16}{\scriptsize $\pm$0.002} & {55.40}{\scriptsize $\pm$0.003} & \\
Vietnam.  &   {43.24}{\scriptsize $\pm$0.002} & {26.96}{\scriptsize $\pm$0.002} & {42.73}{\scriptsize $\pm$0.001} & {42.13}{\scriptsize $\pm$0.002} & \bf {43.34}{\scriptsize $\pm$0.001} & {42.12}{\scriptsize $\pm$0.001} & {42.62}{\scriptsize $\pm$0.003} & \\
\midrule
\multicolumn{3}{l}{\textit{Validation Languages }} & \multicolumn{5}{l}{} \\
Bulgarian  &   {71.19}{\scriptsize $\pm$0.002} & {46.76}{\scriptsize $\pm$0.003} & {78.42}{\scriptsize $\pm$0.003} & {77.62}{\scriptsize $\pm$0.001} & \bf {78.64}{\scriptsize $\pm$0.002} & {78.40}{\scriptsize $\pm$0.001} & {75.30}{\scriptsize $\pm$0.003} & \\
Telugu  &   {64.39}{\scriptsize $\pm$0.018} & {66.78}{\scriptsize $\pm$0.014} & {68.5}{\scriptsize $\pm$0.006} & {64.8}{\scriptsize $\pm$0.008} & \bf {69.91}{\scriptsize $\pm$0.01} & {65.80}{\scriptsize $\pm$0.008} & {67.58}{\scriptsize $\pm$0.008} & \\
\midrule
\multicolumn{3}{l}{\textit{Training Languages }} & \multicolumn{5}{l}{} \\
Arabic  &   {38.53}{\scriptsize $\pm$0.006} & {20.74}{\scriptsize $\pm$0.004} & {71.51}{\scriptsize $\pm$0.002} & {69.76}{\scriptsize $\pm$0.002} & {68.86}{\scriptsize $\pm$0.002} & \bf {73.09}{\scriptsize $\pm$0.002} & {66.40}{\scriptsize $\pm$0.002} & \\
Czech  &   {67.30}{\scriptsize $\pm$0.002} & {43.24}{\scriptsize $\pm$0.002} & {83.15}{\scriptsize $\pm$0.001} & {81.65}{\scriptsize $\pm$0.001} & {82.00}{\scriptsize $\pm$0.001} & \bf {83.21}{\scriptsize $\pm$0.001} & {80.06}{\scriptsize $\pm$0.001} & \\
English  &   \bf {89.29}{\scriptsize $\pm$0.001} & {44.48}{\scriptsize $\pm$0.003} & {82.15}{\scriptsize $\pm$0.004} & {79.48}{\scriptsize $\pm$0.001} & {83.74}{\scriptsize $\pm$0.001} & {81.89}{\scriptsize $\pm$0.001} & {78.04}{\scriptsize $\pm$0.001} & \\
Hindi  &   {35.42}{\scriptsize $\pm$0.002} & \bf {90.99}{\scriptsize $\pm$0.000} & {76.56}{\scriptsize $\pm$0.002} & {74.03}{\scriptsize $\pm$0.004} & {74.15}{\scriptsize $\pm$0.003} & {71.33}{\scriptsize $\pm$0.003} & {74.48}{\scriptsize $\pm$0.004} & \\
Italian  &   {82.50}{\scriptsize $\pm$0.001} & {36.86}{\scriptsize $\pm$0.006} & \bf {87.34}{\scriptsize $\pm$0.002} & {85.28}{\scriptsize $\pm$0.001} & {86.50}{\scriptsize $\pm$0.001} & {87.18}{\scriptsize $\pm$0.002} & {83.09}{\scriptsize $\pm$0.002} & \\
Korean  &   {36.44}{\scriptsize $\pm$0.004} & {40.30}{\scriptsize $\pm$0.002} & {66.35}{\scriptsize $\pm$0.003} & {68.04}{\scriptsize $\pm$0.003} & {63.93}{\scriptsize $\pm$0.003} & \bf {74.08}{\scriptsize $\pm$0.001} & {63.62}{\scriptsize $\pm$0.005} & \\
Norwegian  &   {74.70}{\scriptsize $\pm$0.001} & {43.70}{\scriptsize $\pm$0.003} & {80.09}{\scriptsize $\pm$0.001} & {77.65}{\scriptsize $\pm$0.001} & {78.67}{\scriptsize $\pm$0.001} & \bf {81.33}{\scriptsize $\pm$0.002} & {75.61}{\scriptsize $\pm$0.001} & \\
Russian  &   {68.94}{\scriptsize $\pm$0.003} & {47.29}{\scriptsize $\pm$0.005} & {80.96}{\scriptsize $\pm$0.001} & {79.41}{\scriptsize $\pm$0.001} & {79.93}{\scriptsize $\pm$0.001} & \bf {81.68}{\scriptsize $\pm$0.001} & {76.48}{\scriptsize $\pm$0.002} & \\
\bottomrule
\end{tabular}

==> content/tables/full_s40.tex <==
\begin{tabular}{l|cccccccc}\toprule
%& & & \multicolumn{3}{c|}{$|S|=20$} & \multicolumn{3}{c|}{$|S|=40$} & \multicolumn{3}{c}{$|S|=80$} \\
\textbf{Language} & \textbf{\textsc{en}} & \textbf{\textsc{hin}} & \textbf{\textsc{ne} (EN)} & \textbf{\textsc{ne} (HIN)} & \textbf{\textsc{maml}} & \textbf{\textsc{maml} (HIN)} & \textbf{\MAMLPrime}
\\ \midrule
\multicolumn{3}{l}{\textit{Low-Resource Languages}} & \multicolumn{5}{l}{} \\

Armenian  &   { 50.59}{\scriptsize $\pm$0.005} & { 48.87}{\scriptsize $\pm$0.002} & { 63.54}{\scriptsize $\pm$0.002} & { 63.41}{\scriptsize $\pm$0.004} & { \bf 64.3}{\scriptsize $\pm$0.002} & { 64.17}{\scriptsize $\pm$0.003} & { 59.85}{\scriptsize $\pm$0.004} & \\
Breton  &   { 61.32}{\scriptsize $\pm$0.004} & { 36.09}{\scriptsize $\pm$0.005} & { 61.67}{\scriptsize $\pm$0.005} & { 62.4}{\scriptsize $\pm$0.005} & { \bf 65.12}{\scriptsize $\pm$0.003} & { 62.47}{\scriptsize $\pm$0.004} & { 59.96}{\scriptsize $\pm$0.004} & \\
Buryat  &   { 23.82}{\scriptsize $\pm$0.002} & { 24.71}{\scriptsize $\pm$0.003} & { 25.67}{\scriptsize $\pm$0.003} & { 25.18}{\scriptsize $\pm$0.003} & { 26.38}{\scriptsize $\pm$0.003} & { \bf 26.79}{\scriptsize $\pm$0.003} & { 26.49}{\scriptsize $\pm$0.004} & \\
Faroese  &   { 69.56}{\scriptsize $\pm$0.004} & { 52.3}{\scriptsize $\pm$0.005} & { 68.12}{\scriptsize $\pm$0.006} & { 65.57}{\scriptsize $\pm$0.006} & { \bf 69.88}{\scriptsize $\pm$0.004} & { 67.31}{\scriptsize $\pm$0.003} & { 65.95}{\scriptsize $\pm$0.004} & \\
Kazakh  &   { 47.8}{\scriptsize $\pm$0.004} & { 49.9}{\scriptsize $\pm$0.003} & { 55.08}{\scriptsize $\pm$0.002} & { 53.94}{\scriptsize $\pm$0.003} & { \bf 55.46}{\scriptsize $\pm$0.003} & { 54.45}{\scriptsize $\pm$0.004} & { 54.29}{\scriptsize $\pm$0.005} & \\
U.Sorbian  &   { 50.55}{\scriptsize $\pm$0.005} & { 37.08}{\scriptsize $\pm$0.003} & { 54.7}{\scriptsize $\pm$0.004} & { 53.58}{\scriptsize $\pm$0.003} & { \bf 57.55}{\scriptsize $\pm$0.004} & { 55.64}{\scriptsize $\pm$0.005} & { 52.09}{\scriptsize $\pm$0.005} & \\
\midrule
\multicolumn{3}{l}{\textit{Unseen High-Resource Languages }} & \multicolumn{5}{l}{} \\
Finnish  &   { 56.99}{\scriptsize $\pm$0.003} & { 50.93}{\scriptsize $\pm$0.003} & { 65.07}{\scriptsize $\pm$0.003} & { 64.2}{\scriptsize $\pm$0.004} & { \bf 65.4}{\scriptsize $\pm$0.003} & { 65.05}{\scriptsize $\pm$0.003} & { 62.26}{\scriptsize $\pm$0.004} & \\
French  &   { 65.33}{\scriptsize $\pm$0.002} & { 31.59}{\scriptsize $\pm$0.005} & { 66.59}{\scriptsize $\pm$0.001} & { 64.44}{\scriptsize $\pm$0.002} & { \bf 66.97}{\scriptsize $\pm$0.001} & { 65.68}{\scriptsize $\pm$0.002} & { 63.78}{\scriptsize $\pm$0.003} & \\
German  &   { 72.6}{\scriptsize $\pm$0.001} & { 45.46}{\scriptsize $\pm$0.004} & { 76.17}{\scriptsize $\pm$0.002} & { 74.41}{\scriptsize $\pm$0.002} & { \bf 76.54}{\scriptsize $\pm$0.002} & { 75.23}{\scriptsize $\pm$0.002} & { 74.53}{\scriptsize $\pm$0.003} & \\
Hungarian  &   { 56.23}{\scriptsize $\pm$0.003} & { 46.97}{\scriptsize $\pm$0.004} & { \bf 63.09}{\scriptsize $\pm$0.003} & { 61.33}{\scriptsize $\pm$0.002} & { 62.81}{\scriptsize $\pm$0.002} & { 62.89}{\scriptsize $\pm$0.003} & { 58.09}{\scriptsize $\pm$0.003} & \\
Japanese  &   { 20.05}{\scriptsize $\pm$0.003} & { 43.03}{\scriptsize $\pm$0.006} & { 37.15}{\scriptsize $\pm$0.008} & { 40.56}{\scriptsize $\pm$0.002} & { 42.17}{\scriptsize $\pm$0.004} & { \bf 43.61}{\scriptsize $\pm$0.004} & { 41.51}{\scriptsize $\pm$0.006} & \\
Persian  &   { 44.53}{\scriptsize $\pm$0.004} & { 29.51}{\scriptsize $\pm$0.004} & { 52.76}{\scriptsize $\pm$0.006} & { 53.85}{\scriptsize $\pm$0.004} & { 53.63}{\scriptsize $\pm$0.005} & { \bf 54.0}{\scriptsize $\pm$0.003} & { 50.81}{\scriptsize $\pm$0.004} & \\
Swedish  &   { 80.41}{\scriptsize $\pm$0.001} & { 47.73}{\scriptsize $\pm$0.003} & { 80.81}{\scriptsize $\pm$0.001} & { 79.32}{\scriptsize $\pm$0.002} & { \bf 81.53}{\scriptsize $\pm$0.001} & { 80.14}{\scriptsize $\pm$0.002} & { 77.94}{\scriptsize $\pm$0.002} & \\
Tamil  &   { 32.67}{\scriptsize $\pm$0.004} & { 47.35}{\scriptsize $\pm$0.004} & { 41.72}{\scriptsize $\pm$0.009} & { 39.84}{\scriptsize $\pm$0.004} & { 46.73}{\scriptsize $\pm$0.005} & { 40.84}{\scriptsize $\pm$0.006} & { \bf 48.54}{\scriptsize $\pm$0.008} & \\
Urdu  &   { 26.89}{\scriptsize $\pm$0.005} & { \bf 67.96}{\scriptsize $\pm$0.002} & { 57.36}{\scriptsize $\pm$0.004} & { 50.93}{\scriptsize $\pm$0.004} & { 56.16}{\scriptsize $\pm$0.004} & { 50.16}{\scriptsize $\pm$0.004} & { 55.84}{\scriptsize $\pm$0.003} & \\
Vietnam.  &   { 43.65}{\scriptsize $\pm$0.002} & { 27.92}{\scriptsize $\pm$0.002} & { 42.82}{\scriptsize $\pm$0.002} & { 42.23}{\scriptsize $\pm$0.003} & { \bf 43.74}{\scriptsize $\pm$0.001} & { 42.37}{\scriptsize $\pm$0.001} & { 43.23}{\scriptsize $\pm$0.004} & \\
\midrule
\multicolumn{3}{l}{\textit{Validation Languages }} & \multicolumn{5}{l}{} \\
Bulgarian  &   { 71.21}{\scriptsize $\pm$0.002} & { 47.29}{\scriptsize $\pm$0.004} & { 78.42}{\scriptsize $\pm$0.003} & { 77.62}{\scriptsize $\pm$0.001} & { \bf 78.65}{\scriptsize $\pm$0.002} & { 78.39}{\scriptsize $\pm$0.001} & { 75.44}{\scriptsize $\pm$0.003} & \\
Telugu  &   { 66.64}{\scriptsize $\pm$0.014} & { 67.7}{\scriptsize $\pm$0.013} & { 68.69}{\scriptsize $\pm$0.006} & { 64.75}{\scriptsize $\pm$0.01} & { \bf 70.75}{\scriptsize $\pm$0.012} & { 66.1}{\scriptsize $\pm$0.009} & { 67.97}{\scriptsize $\pm$0.007} & \\
\midrule
\multicolumn{3}{l}{\textit{Training Languages }} & \multicolumn{5}{l}{} \\
Arabic  &   { 41.6}{\scriptsize $\pm$0.012} & { 22.65}{\scriptsize $\pm$0.005} & { 71.53}{\scriptsize $\pm$0.002} & { 69.78}{\scriptsize $\pm$0.002} & { 68.95}{\scriptsize $\pm$0.002} & { \bf 73.01}{\scriptsize $\pm$0.003} & { 66.47}{\scriptsize $\pm$0.002} & \\
Czech  &   { 67.74}{\scriptsize $\pm$0.003} & { 43.92}{\scriptsize $\pm$0.002} & { 83.15}{\scriptsize $\pm$0.001} & { 81.64}{\scriptsize $\pm$0.001} & { 82.03}{\scriptsize $\pm$0.001} & { \bf 83.19}{\scriptsize $\pm$0.001} & { 80.12}{\scriptsize $\pm$0.001} & \\
English  &   { \bf 89.3}{\scriptsize $\pm$0.001} & { 45.32}{\scriptsize $\pm$0.004} & { 82.21}{\scriptsize $\pm$0.004} & { 79.49}{\scriptsize $\pm$0.001} & { 83.96}{\scriptsize $\pm$0.002} & { 82.05}{\scriptsize $\pm$0.002} & { 78.07}{\scriptsize $\pm$0.001} & \\
Hindi  &   { 36.64}{\scriptsize $\pm$0.002} & { \bf 90.99}{\scriptsize $\pm$0.0} & { 76.58}{\scriptsize $\pm$0.002} & { 74.24}{\scriptsize $\pm$0.004} & { 74.28}{\scriptsize $\pm$0.002} & { 72.16}{\scriptsize $\pm$0.004} & { 74.5}{\scriptsize $\pm$0.004} & \\
Italian  &   { 82.68}{\scriptsize $\pm$0.001} & { 38.61}{\scriptsize $\pm$0.007} & { 87.35}{\scriptsize $\pm$0.002} & { 85.28}{\scriptsize $\pm$0.001} & { 86.51}{\scriptsize $\pm$0.001} & { \bf 87.37}{\scriptsize $\pm$0.003} & { 83.11}{\scriptsize $\pm$0.002} & \\
Korean  &   { 36.77}{\scriptsize $\pm$0.004} & { 40.74}{\scriptsize $\pm$0.003} & { 66.4}{\scriptsize $\pm$0.003} & { 68.07}{\scriptsize $\pm$0.003} & { 64.23}{\scriptsize $\pm$0.003} & { \bf 74.01}{\scriptsize $\pm$0.002} & { 63.91}{\scriptsize $\pm$0.004} & \\
Norwegian  &   { 74.7}{\scriptsize $\pm$0.002} & { 44.1}{\scriptsize $\pm$0.006} & { 80.06}{\scriptsize $\pm$0.002} & { 77.53}{\scriptsize $\pm$0.004} & { 78.69}{\scriptsize $\pm$0.001} & { \bf 81.2}{\scriptsize $\pm$0.004} & { 75.64}{\scriptsize $\pm$0.001} & \\
Russian  &   { 69.3}{\scriptsize $\pm$0.003} & { 48.03}{\scriptsize $\pm$0.005} & { 80.98}{\scriptsize $\pm$0.001} & { 79.43}{\scriptsize $\pm$0.001} & { 80.0}{\scriptsize $\pm$0.001} & { \bf 81.66}{\scriptsize $\pm$0.001} & { 76.57}{\scriptsize $\pm$0.002} & \\

\bottomrule
\end{tabular}

==> content/tables/full_s80.tex <==
\begin{tabular}{l|cccccccc}\toprule
%& & & \multicolumn{3}{c|}{$|S|=20$} & \multicolumn{3}{c|}{$|S|=40$} & \multicolumn{3}{c}{$|S|=80$} \\
\textbf{Language} & \textbf{\textsc{en}} & \textbf{\textsc{hin}} & \textbf{\textsc{ne} (EN)} & \textbf{\textsc{ne} (HIN)} & \textbf{\textsc{maml}} & \textbf{\textsc{maml} (HIN)} & \textbf{\MAMLPrime}
\\ \midrule
\multicolumn{3}{l}{\textit{Low-Resource Languages}} & \multicolumn{5}{l}{} \\

Armenian  &   { 51.99}{\scriptsize $\pm$0.005} & { 49.7}{\scriptsize $\pm$0.002} & { 63.79}{\scriptsize $\pm$0.002} & { 63.59}{\scriptsize $\pm$0.004} & { \bf 64.78}{\scriptsize $\pm$0.003} & { 64.76}{\scriptsize $\pm$0.003} & { 60.03}{\scriptsize $\pm$0.003} \\
Breton  &   { 62.76}{\scriptsize $\pm$0.004} & { 38.95}{\scriptsize $\pm$0.004} & { 62.2}{\scriptsize $\pm$0.006} & { 63.05}{\scriptsize $\pm$0.004} & { \bf 66.14}{\scriptsize $\pm$0.003} & { 63.75}{\scriptsize $\pm$0.004} & { 60.84}{\scriptsize $\pm$0.004} \\
Buryat  &   { 24.17}{\scriptsize $\pm$0.003} & { 25.54}{\scriptsize $\pm$0.003} & { 25.88}{\scriptsize $\pm$0.003} & { 25.4}{\scriptsize $\pm$0.003} & { 27.33}{\scriptsize $\pm$0.003} & { \bf 27.37}{\scriptsize $\pm$0.004} & { 27.05}{\scriptsize $\pm$0.004} \\
Faroese  &   { 70.59}{\scriptsize $\pm$0.004} & { 54.64}{\scriptsize $\pm$0.005} & { 68.62}{\scriptsize $\pm$0.006} & { 66.17}{\scriptsize $\pm$0.005} & { \bf 71.12}{\scriptsize $\pm$0.004} & { 68.25}{\scriptsize $\pm$0.003} & { 66.79}{\scriptsize $\pm$0.004} \\+
Kazakh  &   { 49.08}{\scriptsize $\pm$0.004} & { 50.49}{\scriptsize $\pm$0.003} & { 55.23}{\scriptsize $\pm$0.003} & { 54.08}{\scriptsize $\pm$0.003} & { \bf 56.15}{\scriptsize $\pm$0.003} & { 55.0}{\scriptsize $\pm$0.004} & { 54.99}{\scriptsize $\pm$0.005} \\
U.Sorbian  &   { 52.11}{\scriptsize $\pm$0.005} & { 38.22}{\scriptsize $\pm$0.004} & { 55.08}{\scriptsize $\pm$0.004} & { 53.94}{\scriptsize $\pm$0.004} & { \bf 58.78}{\scriptsize $\pm$0.005} & { 56.56}{\scriptsize $\pm$0.006} & { 52.38}{\scriptsize $\pm$0.005} \\
\midrule
\multicolumn{3}{l}{\textit{Unseen High-Resource Languages }} & \multicolumn{5}{l}{} \\
Finnish  &   { 57.73}{\scriptsize $\pm$0.004} & { 51.79}{\scriptsize $\pm$0.002} & { 65.18}{\scriptsize $\pm$0.003} & { 64.4}{\scriptsize $\pm$0.004} & { \bf 65.82}{\scriptsize $\pm$0.005} & { 65.61}{\scriptsize $\pm$0.004} & { 62.47}{\scriptsize $\pm$0.004} \\
French  &   { 65.63}{\scriptsize $\pm$0.002} & { 33.39}{\scriptsize $\pm$0.006} & { 66.65}{\scriptsize $\pm$0.001} & { 64.42}{\scriptsize $\pm$0.002} & { \bf 67.25}{\scriptsize $\pm$0.002} & { 65.69}{\scriptsize $\pm$0.003} & { 64.15}{\scriptsize $\pm$0.003} \\
German  &   { 72.93}{\scriptsize $\pm$0.002} & { 46.65}{\scriptsize $\pm$0.003} & { 76.21}{\scriptsize $\pm$0.002} & { 74.46}{\scriptsize $\pm$0.002} & { \bf 76.72}{\scriptsize $\pm$0.002} & { 75.31}{\scriptsize $\pm$0.002} & { 74.72}{\scriptsize $\pm$0.003} \\
Hungarian  &   { 56.73}{\scriptsize $\pm$0.003} & { 47.91}{\scriptsize $\pm$0.003} & { \bf 63.21}{\scriptsize $\pm$0.003} & { 61.68}{\scriptsize $\pm$0.002} & { 62.52}{\scriptsize $\pm$0.002} & { 62.91}{\scriptsize $\pm$0.002} & { 57.48}{\scriptsize $\pm$0.004} \\
Japanese  &   { 22.8}{\scriptsize $\pm$0.004} & { \bf 46.87}{\scriptsize $\pm$0.004} & { 38.4}{\scriptsize $\pm$0.007} & { 41.58}{\scriptsize $\pm$0.003} & { 46.81}{\scriptsize $\pm$0.003} & { 45.9}{\scriptsize $\pm$0.004} & { 43.87}{\scriptsize $\pm$0.005} \\
Persian  &   { 46.42}{\scriptsize $\pm$0.006} & { 31.11}{\scriptsize $\pm$0.01} & { 53.11}{\scriptsize $\pm$0.006} & { 54.06}{\scriptsize $\pm$0.004} & { \bf 54.74}{\scriptsize $\pm$0.006} & { 54.53}{\scriptsize $\pm$0.005} & { 51.08}{\scriptsize $\pm$0.004} \\
Swedish  &   { 80.57}{\scriptsize $\pm$0.001} & { 49.15}{\scriptsize $\pm$0.002} & { 80.79}{\scriptsize $\pm$0.002} & { 79.31}{\scriptsize $\pm$0.002} & { \bf 81.59}{\scriptsize $\pm$0.001} & { 80.21}{\scriptsize $\pm$0.002} & { 78.1}{\scriptsize $\pm$0.002} \\
Tamil  &   { 34.81}{\scriptsize $\pm$0.007} & { 48.55}{\scriptsize $\pm$0.002} & { 42.88}{\scriptsize $\pm$0.008} & { 40.73}{\scriptsize $\pm$0.004} & { \bf 50.68}{\scriptsize $\pm$0.003} & { 42.81}{\scriptsize $\pm$0.006} & { 50.54}{\scriptsize $\pm$0.008} \\
Urdu  &   { 29.3}{\scriptsize $\pm$0.004} & { \bf 68.17}{\scriptsize $\pm$0.004} & { 57.63}{\scriptsize $\pm$0.004} & { 51.5}{\scriptsize $\pm$0.004} & { 57.6}{\scriptsize $\pm$0.004} & { 51.57}{\scriptsize $\pm$0.004} & { 56.28}{\scriptsize $\pm$0.004} \\
Vietnam.  &   { 44.28}{\scriptsize $\pm$0.002} & { 29.61}{\scriptsize $\pm$0.002} & { 42.99}{\scriptsize $\pm$0.002} & { 42.46}{\scriptsize $\pm$0.003} & { \bf 44.33}{\scriptsize $\pm$0.002} & { 42.88}{\scriptsize $\pm$0.002} & { 43.78}{\scriptsize $\pm$0.004} \\
\midrule
\multicolumn{3}{l}{\textit{Validation Languages }} & \multicolumn{5}{l}{} \\
Bulgarian  &   { 71.42}{\scriptsize $\pm$0.003} & { 48.07}{\scriptsize $\pm$0.006} & { 78.43}{\scriptsize $\pm$0.003} & { 77.67}{\scriptsize $\pm$0.002} & { \bf 78.67}{\scriptsize $\pm$0.003} & { 78.45}{\scriptsize $\pm$0.002} & { 75.68}{\scriptsize $\pm$0.003} \\
Telugu  &   { 69.08}{\scriptsize $\pm$0.011} & { 68.79}{\scriptsize $\pm$0.01} & { 68.97}{\scriptsize $\pm$0.006} & { 65.05}{\scriptsize $\pm$0.009} & { \bf 71.52}{\scriptsize $\pm$0.012} & { 66.86}{\scriptsize $\pm$0.008} & { 68.41}{\scriptsize $\pm$0.008} \\
\midrule
\multicolumn{3}{l}{\textit{Training Languages }} & \multicolumn{5}{l}{} \\
Arabic  &   { 46.24}{\scriptsize $\pm$0.015} & { 25.5}{\scriptsize $\pm$0.006} & { 71.54}{\scriptsize $\pm$0.002} & { 69.79}{\scriptsize $\pm$0.002} & { 69.07}{\scriptsize $\pm$0.002} & { \bf 73.04}{\scriptsize $\pm$0.002} & { 66.51}{\scriptsize $\pm$0.002} \\
Czech  &   { 68.4}{\scriptsize $\pm$0.003} & { 45.28}{\scriptsize $\pm$0.002} & { 83.16}{\scriptsize $\pm$0.001} & { 81.65}{\scriptsize $\pm$0.001} & { 82.04}{\scriptsize $\pm$0.001} & { \bf 83.2}{\scriptsize $\pm$0.001} & { 80.15}{\scriptsize $\pm$0.001} \\
English  &   { \bf 89.3}{\scriptsize $\pm$0.001} & { 46.87}{\scriptsize $\pm$0.002} & { 82.32}{\scriptsize $\pm$0.003} & { 79.51}{\scriptsize $\pm$0.001} & { 84.28}{\scriptsize $\pm$0.002} & { 82.08}{\scriptsize $\pm$0.002} & { 78.07}{\scriptsize $\pm$0.002} \\
Hindi  &   { 39.25}{\scriptsize $\pm$0.003} & { \bf 90.96}{\scriptsize $\pm$0.0} & { 76.61}{\scriptsize $\pm$0.002} & { 74.65}{\scriptsize $\pm$0.004} & { 74.46}{\scriptsize $\pm$0.003} & { 73.3}{\scriptsize $\pm$0.003} & { 74.63}{\scriptsize $\pm$0.004} \\
Italian  &   { 82.96}{\scriptsize $\pm$0.001} & { 41.8}{\scriptsize $\pm$0.009} & { 87.35}{\scriptsize $\pm$0.002} & { 85.29}{\scriptsize $\pm$0.001} & { 86.57}{\scriptsize $\pm$0.002} & { \bf 87.39}{\scriptsize $\pm$0.003} & { 83.17}{\scriptsize $\pm$0.002} \\
Korean  &   { 37.77}{\scriptsize $\pm$0.005} & { 41.53}{\scriptsize $\pm$0.003} & { 66.46}{\scriptsize $\pm$0.003} & { 68.16}{\scriptsize $\pm$0.003} & { 64.36}{\scriptsize $\pm$0.004} & { \bf 74.05}{\scriptsize $\pm$0.002} & { 64.21}{\scriptsize $\pm$0.005} \\
Norwegian  &   { 74.93}{\scriptsize $\pm$0.002} & { 45.3}{\scriptsize $\pm$0.004} & { 80.08}{\scriptsize $\pm$0.002} & { 77.56}{\scriptsize $\pm$0.004} & { 78.76}{\scriptsize $\pm$0.001} & { \bf 81.22}{\scriptsize $\pm$0.004} & { 75.69}{\scriptsize $\pm$0.001} \\
Russian  &   { 69.79}{\scriptsize $\pm$0.003} & { 49.02}{\scriptsize $\pm$0.004} & { 81.01}{\scriptsize $\pm$0.001} & { 79.45}{\scriptsize $\pm$0.001} & { 80.04}{\scriptsize $\pm$0.001} & { \bf 81.67}{\scriptsize $\pm$0.001} & { 76.56}{\scriptsize $\pm$0.002} \\

\bottomrule
\end{tabular}

==> content/tables/mamlresults.tex <==
\begin{tabular}{l|rr|rr|rr}
\toprule
& \multicolumn{2}{c|}{$|S| = 20$} & \multicolumn{2}{c|}{$|S| = 40$} & \multicolumn{2}{c}{$|S| = 80$} \\
\textbf{Language} & \textbf{\textsc{maml}} & \textbf{\MAMLPrime} & \textbf{\textsc{maml}} & \textbf{\MAMLPrime} & \textbf{\textsc{maml}} & \textbf{\MAMLPrime} \\
\midrule
\multicolumn{3}{l|}{\textit{Low-Resource Languages}} & \multicolumn{2}{l|}{} & \multicolumn{2}{l}{} \\
Armenian        &\bf\underline{63.84} & 59.70 &\bf\underline{64.30} & 59.85 & \bf\underline{64.78} & 60.03 \\
Breton          &\bf\underline{64.18} & 59.33 &\bf\underline{65.12} & 59.96 & \bf\underline{66.14} & 60.84 \\
Buryat$\dagger$& 25.77 & \bf 26.02 & 26.38 &\bf 26.49 & \bf 27.33 & 27.05 \\
Faroese$\dagger$&\bf\underline{68.95}& 65.30 &\bf\underline{69.88} & 65.95 & \bf\underline{71.12} & 66.79 \\
Kazakh          &\bf\underline{55.07} & 53.92 &\bf\underline{55.46} & 54.29 & \bf\underline{56.15} & 54.99 \\
U.Sorbian$\dagger$&\bf\underline{56.40} & 51.67 & \bf\underline{57.55} & 52.09 & \bf\underline{58.78} & 52.38 \\\midrule
\multicolumn{3}{l|}{\textit{High-Resource Languages}} & \multicolumn{2}{l|}{} & \multicolumn{2}{l}{} \\
Finnish         &\bf\underline{64.89} & 61.97 & \bf\underline{65.40} & 62.26 & \bf\underline{65.82} & 62.47 \\
French          &\bf\underline{66.85} & 63.42 & \bf\underline{66.97} & 63.78 & \bf\underline{67.25} & 64.15 \\
German          &\bf\underline{76.41} & 74.38 & \bf\underline{76.54} & 74.53 & \bf\underline{76.72} & 74.72 \\
Hungarian       &\bf\underline{62.71} & 58.47 & \bf\underline{62.81} & 58.09 & \bf\underline{62.52} & 57.48 \\
Japanese        & 39.06 & \bf 39.72 & \bf 42.17 & 41.51 & \bf\underline{46.81} & 43.87 \\
Persian         &\bf\underline{52.81} & 50.31 & \bf\underline{53.63} & 50.81 & \bf\underline{54.74} & 51.08 \\
Swedish         &\bf\underline{81.36} & 77.57 & \bf\underline{81.53} & 77.94 & \bf\underline{81.59} & 78.10 \\
Tamil           & 44.34   &\bf\underline{46.55} & 46.73 & \bf\underline{48.54} & \bf 50.68 & 50.54 \\
Urdu            & 55.16   & \bf 55.4 & \bf 56.16 & 55.84 & \bf\underline{57.60} & 56.28 \\
Vietnamese      &\bf 43.34& 42.62 &\bf 43.74 & 43.23 & \bf\underline{44.33} & 43.78 \\
\bottomrule
\end{tabular}
  
%\begin{tabular}{|l|rr|rr|rr|}\hline
%Language & Few-Shot \\\hline
%& \multicolumn{2}{c|}{$|S| = 20$} & \multicolumn{2}{c|}{$|S| = 40$} & \multicolumn{2}{c|}{$|S| = 80$} \\\hline
%& MAML & MAML' & MAML & MAML' & MAML & MAML' \\ \hline
% Armenian  &   { \bf 63.84}* & { 59.7} & { \bf 64.3}* & { 59.85} & { \bf 64.78}* & { 60.03} \\
% Breton  &   { \bf 64.18}* & { 59.33} & { \bf 65.12}* & { 59.96} & { \bf 66.14}* & { 60.84} \\
% Buryat$^\dagger$  &   { 25.77} & { \bf 26.02} & { 26.38} & { \bf 26.49} & { \bf 27.33} & { 27.05} \\
% Faroese$^\dagger$  &   { \bf 68.95}* & { 65.3} & { \bf 69.88}* & { 65.95} & { \bf 71.12}* & { 66.79} \\
% Kazakh  &   { \bf 55.07}* & { 53.92} & { \bf 55.46}* & { 54.29} & { \bf 56.15}* & { 54.99} \\
% U.Sorbian$^\dagger$  &   { \bf 56.4}* & { 51.67} & { \bf 57.55}* & { 52.09} & { \bf 58.78}* & { 52.38} \\\hline
% Finnish  &   { \bf 64.89}* & { 61.97} & { \bf 65.4}* & { 62.26} & { \bf 65.82}* & { 62.47} \\
% French  &   { \bf 66.85}* & { 63.42} & { \bf 66.97}* & { 63.78} & { \bf 67.25}* & { 64.15} \\
% German  &   { \bf 76.41}* & { 74.38} & { \bf 76.54}* & { 74.53} & { \bf 76.72}* & { 74.72} \\
% Hungarian  &   { \bf 62.71}* & { 58.47} & { \bf 62.81}* & { 58.09} & { \bf 62.52}* & { 57.48} \\
% Japanese  &   { 39.06} & { \bf 39.72} & { \bf 42.17} & { 41.51} & { \bf 46.81}* & { 43.87} \\
% Persian  &   { \bf 52.81}* & { 50.31} & { \bf 53.63}* & { 50.81} & { \bf 54.74}* & { 51.08} \\
% Swedish  &   { \bf 81.36}* & { 77.57} & { \bf 81.53}* & { 77.94} & { \bf 81.59}* & { 78.1} \\
% Tamil  &   { 44.34} & { \bf 46.55}* & { 46.73} & { \bf 48.54}* & { \bf 50.68} & { 50.54} \\
% Urdu  &   { 55.16} & { \bf 55.4} & { \bf 56.16} & { 55.84} & { \bf 57.6}* & { 56.28} \\
% Vietnamese  &   { \bf 43.34} & { 42.62} & { \bf 43.74} & { 43.23} & { \bf 44.33}* & { 43.78} \\
%\hline
%\end{tabular}

==> content/tables/mamlresultshindi.tex <==
\begin{tabular}{l|rr|rr|rr}\toprule
& \multicolumn{2}{c|}{$|S| = 20$} & \multicolumn{2}{c|}{$|S| = 40$} & \multicolumn{2}{c}{$|S| = 80$} \\
\bf Language    & \bf \textsc{maml} & \bf \MAMLPrime & \bf \textsc{maml} & \bf \MAMLPrime & \bf \textsc{maml} & \bf \MAMLPrime \\ \midrule
\multicolumn{3}{l|}{\textit{Low-Resource Languages}} & \multicolumn{2}{l|}{} & \multicolumn{2}{l}{} \\
Armenian  		&  \bf \underline{63.76} & {59.7}  & \bf \underline{64.17} & {59.85} & \bf \underline{64.76} & {60.03} \\
Breton  		&  \bf \underline{61.56} & {59.33} & \bf \underline{62.47} & {59.96} & \bf \underline{63.75} & {60.84} \\
Buryat$\dagger$ &  \bf {26.27} & {26.02} & \bf {26.79} & {26.49} & \bf {27.37} & {27.05} \\
Faroese$\dagger$&  \bf {66.82} & {65.30} & \bf \underline{67.31} & {65.95} & \bf \underline{68.25} & {66.79} \\
Kazakh  		&  \bf {54.23} & {53.92} & \bf {54.45} & {54.29} & \bf {55.00} & {54.99} \\
U.Sorbian$\dagger$ &   \bf \underline{54.97} & {51.67} & \bf \underline{55.64} & {52.09} & \bf \underline{56.56} & {52.38} \\\midrule
\multicolumn{3}{l|}{\textit{High-Resource Languages}} & \multicolumn{2}{l|}{} & \multicolumn{2}{l}{} \\
Finnish  		& \bf \underline{64.64} & {61.97} & \bf \underline{65.05} & {62.26} & \bf \underline{65.61} & {62.47} \\
French  		& \bf \underline{65.73} & {63.42} & \bf \underline{65.68} & {63.78} & \bf \underline{65.69} & {64.15} \\
German  		& \bf {75.15} & {74.38} & \bf \underline{75.23} & {74.53} & \bf \underline{75.31} & {74.72} \\
Hungarian  		& \bf \underline{62.51} & {58.47} & \bf \underline{62.89} & {58.09} & \bf \underline{62.91} & {57.48} \\
Japanese  		& \bf \underline{41.96} & {39.72} & \bf \underline{43.61} & {41.51} & \bf \underline{45.90} & {43.87} \\
Persian  		& \bf \underline{53.63} & {50.31} & \bf \underline{54.0} & {50.81} & \bf \underline{54.53} & {51.08} \\
Swedish  		& \bf \underline{79.89} & {77.57} & \bf \underline{80.14} & {77.94} & \bf \underline{80.21} & {78.10} \\
Tamil  			& {39.57} & \bf \underline{46.55} & {40.84} & \bf \underline{48.54} & {42.81} & \bf \underline{50.54} \\
Urdu  			& {49.16} & \bf \underline{55.40} & {50.16} & \bf \underline{55.84} & {51.57} & \bf \underline{56.28} \\
Vietnamese  	& {42.12} & \bf {42.62} & {42.37} & \bf \underline{43.23} & {42.88} & \bf \underline{43.78} \\
\bottomrule
\end{tabular}

==> content/tables/projectivity_stats.tex <==
\begin{tabular}{l|r}\toprule
    \bf Language & \bf Percentage \\\midrule
    Telugu & 0.002\\
    %Chinese-GSD &0.007\\
    Italian &0.021\\
    %Amharic-ATT &0.024\\
    Japanese & 0.026\\
    Breton & 0.027\\
    Faroese & 0.027\\
    Tamil & 0.028\\
    Vietnamese & 0.029\\
    Bulgarian & 0.031\\
    %Bambara-CRB&0.032\\
    Swedish & 0.038\\
    English & 0.048\\
   % Uyghur-UDT &0.05\\
    French & 0.055\\
    Finnish & 0.063\\
    Persian & 0.067\\
    Russian & 0.08\\
    %Erzya-JR & 0.082\\
    Norwegian & 0.082\\
    %Cantonese-HK &0.086\\
    German & 0.092\\
    Arabic & 0.092\\
    Armenian & 0.102\\
    Upper Sorbian & 0.113\\
   % Turkish-IMST& 0.115 \\
    Czech & 0.119\\
    Kazakh & 0.121\\
    Hindi & 0.136\\
    Buryat & 0.156\\
    Korean & 0.217\\
    Urdu & 0.226\\
    Hungarian & 0.271\\
    %Basque-BDT & 0.332\\
    \bottomrule
  \end{tabular}
